Neural Implicit Solution Formula for Efficiently Solving Hamilton-Jacobi Equations

This paper presents an implicit solution formula for the Hamilton-Jacobi partial differential equation (HJ PDE). The formula is derived using the method of characteristics and is shown to coincide with the Hopf and Lax formulas in the case where either the Hamiltonian or the initial function is convex. It provides a simple and efficient numerical approach for computing the viscosity solution of HJ PDEs, bypassing the need for the Legendre transform of the Hamiltonian or the initial condition, and the explicit computation of individual characteristic trajectories. A deep learning-based methodology is proposed to learn this implicit solution formula, leveraging the mesh-free nature of deep learning to ensure scalability for high-dimensional problems. Building upon this framework, an algorithm is developed that approximates the characteristic curves piecewise linearly for state-dependent Hamiltonians. Extensive experimental results demonstrate that the proposed method delivers highly accurate solutions, even for nonconvex Hamiltonians, and exhibits remarkable scalability, achieving computational efficiency for problems up to 40 dimensions.

==> sub.tex <==
% This paper derives a novel implicit solution formula for Hamilton-Jacobi equations. By effectively combining it with deep learning techniques, we propose a simple yet highly efficient deep learning-based methodology that enables the scalable handling of complex and high-dimensional problems.

% We believe this paper is of broad interest to SISC readers as it combines mathematical derivations with efficient deep learning methods, covering both theoretical and practical aspects.

% By deriving a new solution formula for the Hamilton-Jacobi equation, this approach is fundamentally distinct from existing research.

% We would like to recommend the following individuals as potential editors or reviewers for our manuscript, based on their expertise in the relevant field:

% Lars Ruthotto, Emory University (lruthotto@emory.edu)
% Bin Dong, Peking University (dongbin@math.pku.edu.cn)
% Tao Tang, BNU-HKBU United International College (ttang@uic.edu.cn)
